Oscillation mode linewidths and heights of 23 main-sequence stars observed by Kepler

Solar-like oscillations have been observed by Kepler and CoRoT in many solar-type stars, thereby providing a way to probe the stars using asteroseismology. We provide the mode linewidths and mode heights of the oscillations of various stars as a function of frequency and of effective temperature. We used a time series of nearly two years of data for each star. The 23 stars observed belong to the simple or F-like category. The power spectra of the 23 main-sequence stars were analysed using both maximum likelihood estimators and Bayesian estimators, providing individual mode characteristics such as frequencies, linewidths, and mode heights. We study the source of systematic errors in the mode linewidths and mode heights, and we present a way to correct these errors with respect to a common reference fit. Using the correction, we could explain all sources of systematic errors, which could be reduced to less than $\pm$15% for mode linewidths and heights, and less than $\pm$5% for amplitude, when compared to the reference fit. The effect of a different estimated stellar background and a different estimated splitting will provide frequency-dependent systematic errors that might affect the comparison with theoretical mode linewidth and mode height, therefore affecting the understanding of the physical nature of these parameters. All other sources of relative systematic errors are less dependent upon frequency. We also provide the dependence of the so-called linewidth dip, in the middle of the observed frequency range, as a function of effective temperature. We show that the depth of the dip decreases with increasing effective temperature. The dependence of the dip on effective temperature may imply that the mixing length parameter $\alpha$ or the convective flux may increase with effective temperature.

==> table_linewidth.tex <==
\begin{table*}[!]
\caption{Table of key stellar parameters.  The first three columns provide the KIC, HIP, and HD numbers.  The fourth column provides the effective temperature and its error bar taken from \citet{Pins2011}.  The fifth column provides the {\it Kepler} magnitude.  The sixth column gives the median of the large separation as measured using the mode frequencies given in this paper.  The seventh column provides the frequency of the maximum of oscillation power.  The eighth column gives the star category as provided by \citet{Appourchaux2012}.  The  penultimate column gives the duration of observation.  The last column provides the start and end quarter of the observation.}
\centering
\begin{tabular}{r r r c r r r c c c} 
\hline
\hline
KIC&HIP&HD&$T_{\rm eff}$ (K)&Kp& $\Delta\nu$ ($\mu$Hz)&$\nu_{\rm max}$($\mu$Hz) &Star category&Duration (in months)&Quarters\\
\hline
\hline
1435467&-&-&        6541 $\pm$         126&8.9&70.9&1324&F-like&24&Q5-Q12\\
2837475&-&-&        6710 $\pm$          61&8.5&76.0&1522&F-like&24&Q5-Q12\\
3424541&-&-&        6460 $\pm$          55&9.7&41.3&712&F-like&24&Q5-Q12\\
3733735&94071&178971&        6720 $\pm$          56&8.4&92.4&2041&F-like&24&Q5-Q12\\
6116048&-&-&        6020 $\pm$          51&8.4&100.7&2020&simple&24&Q5-Q12\\
6508366&-&-&        6480 $\pm$          56&9.0&51.6&959&F-like&24&Q5-Q12\\
6679371&-&-&        6590 $\pm$          56&8.7&50.4&908&F-like&24&Q5-Q12\\
7103006&-&-&        6390 $\pm$          56&8.9&59.9&1072&F-like&24&Q5-Q12\\
7206837&-&-&        6360 $\pm$          56&9.8&79.0&1556&simple&24&Q5-Q12\\
8379927&97321&187160&        5990 $\pm$          52&7.0&120.4&2669&simple&24&Q5-Q12\\
8694723&-&-&        6310 $\pm$          56&8.9&75.1&1384&simple&24&Q5-Q12\\
9139151&92961&-&        6090 $\pm$          52&9.2&117.0&2610&simple&24&Q5-Q12\\
9139163&92962&-&        6370 $\pm$          56&8.3&81.4&1649&simple&24&Q5-Q12\\
9206432&93607&-&        6470 $\pm$          56&9.1&85.1&1822&F-like&24&Q5-Q12$\,^{a}$\\
9812850&-&-&        6380 $\pm$          55&9.5&65.3&1186&F-like&24&Q5-Q12\\
10162436&97992&-&        6320 $\pm$          53&8.6&55.9&1004&simple&24&Q5-Q12$\,^{b}$\\
10355856&-&-&        6540 $\pm$          56&9.2&68.3&1210&F-like&15&Q5-Q9$\,^{c}$\\
10454113&92983&-&        6246 $\pm$          58&8.6&105.2&2313&simple&24&Q5-Q12\\
10909629&-&-&        6490 $\pm$          61&10.9&49.7&813&F-like&21&Q5-Q11$\,^{d}$\\
11081729&-&-&        6600 $\pm$          62&9.0&90.2&1820&F-like&24&Q5-Q12\\
12009504&-&-&        6230 $\pm$          51&9.3&88.1&1768&simple&24&Q5-Q12\\
12258514&95568&183298&        5950 $\pm$          51&8.1&74.8&1449&simple&24&Q5-Q12\\
12317678&97316&-&        6540 $\pm$          55&8.7&64.1&1162&F-like&24&Q5-Q12\\
\hline
\end{tabular}
\begin{list}{}{}
\item[$^{\rm a}$] Q7 missing.
\item[$^{\rm b}$] Q7, Q10, Q11 missing.
\item[$^{\rm c}$] Q7 missing.
\item[$^{\rm d}$] Q8, Q9, Q10 missing.
\end{list}
\end{table*}

